PI-Whisper: Designing an Adaptive and Incremental Automatic Speech Recognition System for Edge Devices

Edge-based automatic speech recognition (ASR) technologies are increasingly prevalent in the development of intelligent and personalized assistants. However, resource-constrained ASR models face significant challenges in adaptivity, incrementality, and inclusivity when faced with a diverse population. To tackle those challenges, we propose PI-Whisper, a novel ASR system that adaptively enhances recognition capabilities by identifying speakers' characteristics in real-time. In this work, we show how the design of PI-Whisper allows for incremental adaptation of new characteristics without the need for repetitive retraining, enhances recognition capabilities, and improves equity and fairness across diverse speaker groups. PI-Whisper demonstrates these advantages by achieving state-of-the-art accuracy, reducing the word error rate (WER) by up to 13.7% relative to baselines while scaling linearly to computing resources.

==> 0_abstract.tex <==
% \begin{abstract}
% State-of-the-art ASR models are often deployed statically on the cloud. To utilize their services, users are required to upload their data for inference, which poses a privacy concern. Such a concern requires us to deploy models on computationally constrained local edge devices to ensure full user control, but that approach poses the challenge of balancing model miniaturization, accuracy, and adaptability to diverse populations. Existing works fail on either privacy-preserving edge deployment or sustainability to adapt to progressively increased diversity demands. To address the above challenges, we propose \textbf{P-Whisper}, which features low computational requirements, dynamic adaptation, and no need for repetitive model training.  P-Whisper utilizes the merging of LoRA profiles tailored to the characteristics of different populations.
% \end{abstract}

\begin{abstract}
State-of-the-art ASR models are often deployed statically on the cloud, which requires users to upload their data for inference, posing a privacy concern. Such concern requires us to deploy models on resource-constrained local edge devices, which poses the challenge of balancing model deployment feasibility, accuracy, and adaptability to diverse populations. Existing works fail on either privacy-preserving edge deployment or sustainability to adapt to progressively increased diversity demands. In this paper, we propose \textbf{P-Whisper}, a lightweight framework that features low computational requirements, dynamic adaptation, and no need for repetitive model re-training.  P-Whisper utilizes the merging of multiple LoRA profiles tailored to the characteristics of different populations to enhance ASR performance. Our experiments demonstrate that P-Whisper achieves accurate and fair adaptation on people of different ages, accents, and genders with very low training and inference overhead.
\end{abstract}

==> 0_abstract_JX.tex <==
\begin{abstract}
As edge-based automatic speech recognition (ASR) technologies become increasingly prevalent for the development of intelligent and personalized assistants, three important challenges must be addressed for these resource-constrained ASR models, i.e., adaptivity, incrementality, and inclusivity. We propose a novel ASR framework, PI-Whisper, in this work and show how it can improve an ASR’s recognition capabilities adaptively by identifying different speakers’ characteristics in real-time, how such an adaption can be performed incrementally without repetitive retraining, and how it can improve the equity and fairness for diverse speaker groups. More impressively, our proposed PI-Whisper framework attains all of these nice properties while still achieving state-of-the-art accuracy with up to 13.7\% reduction of the word error rate (WER) with linear scalability with respect to computing resources.
\end{abstract}

==> 0_abstract_v1.tex <==
\begin{abstract}
State-of-the-art ASR models are often deployed statically on the cloud. To utilize their services, users are required to upload their data for inference, which poses a privacy concern. Such a concern requires us to deploy models on computationally constrained local edge devices to ensure full user control, but that approach poses the challenge of balancing model miniaturization, accuracy, and adaptability to diverse populations. Existing works fail on either privacy-preserving edge deployment or sustainability to adapt to progressively increased diversity demands. To address the above challenges, we propose \textbf{P-Whisper}, which features low computational requirements, dynamic adaptation, and no need for repetitive model training.  P-Whisper utilizes the merging of LoRA profiles tailored to the characteristics of different populations.
\end{abstract}

==> 1_intro.tex <==
\section{Introduction}
%\textcolor{red}{NEED to rewrite the story}

The advances in deep learning have brought unprecedented improvement in the field of automatic speech recognition (ASR). Recent works such as Whisper and its variants \cite{radford2022robust,bain23_interspeech} have demonstrated remarkable accuracy and robustness in recognizing speech across various languages, accents, and noisy environments. However, despite these advancements, significant challenges remain in attaining privacy and diversity concerns when adapting and deploying these models in real-world applications. 


The first concern when deploying ASR models is the preservation of the privacy of data used in both training and inference. This requirement is crucial when the ASR's task is to transcribe and analyze audio samples from sensitive subjects who do not wish to disclose any sensitive or private information \citep{ahmed2020preech,liu2022private}. 
Tackling this challenge usually involves cutting the ASR's connection to the cloud and deploying the model on local edge devices \citep{ahmed2020preech,liu2022private}. Those devices often have constrained computational power and resources, which limits the capabilities of deploying large ASR models that utilize an extensive amount of resources. However, while smaller models could be trained and perform real-time inference on the edge, they are not expressive enough to perform those tasks accurately. This presents the challenge of balancing model accuracy with deployment feasibility.

%However, despite these advancements, there remain significant challenges in adapting these models to diverse populations, particularly when considering the computational constraints of deployment on edge devices.
 %One of the foremost practical challenges in ASR today is the balance between model accuracy and deployment feasibility. Arguably, transformer models more-or-less all follow the scaling law \citep{kaplan2020scaling}, which states that the performance of a model is positively related to its size. This behavior is also observable in ASR models, the larger the model is, the better the yield performance is. This is due to the model's capacity to capture complex linguistic patterns and variations. As shown in Figure \ref{fig:libri}, the performance of different \amir{??variations??} of the Whisper family \citep{radford2022robust} on two benchmarks \citep{librispeech, Heikinheimo_2023} indicates that larger models achieve higher quality transcriptions with lower word error rates (WER). \amir{Increasing the parameter size requires more training hours and data, which are a rare commodity.

 %}



% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{latex/_fig/librispeech.png}
%     \caption{Different sizes of Whisper model's performance on Librispeech (clean) dataset's test split.}
%     \label{fig:libri}
% \end{figure}


% Nonetheless, in scenarios where the privacy of training and inference data is valued, these large and powerful models are often too resource-intensive to be deployed on local edge devices, which have limited computational power and resources \citep{qin2024empirical}. For example, when the ASR tasks involve transcribing and analyzing audio samples from sensitive subjects who do not wish to disclose their speech \citep{ahmed2020preech,liu2022private}, large ASR models that are running on cloud computation infrastructures could not be used, and we will have to consider smaller models that are not as expressive yet fit into edge devices. 

%\amir{We need to emphasize the use case of edge more}

 % Another difficulty faced is making the ASR inclusive to a more diverse population.
 % Datasets that are used for training are usually collected from a small sample of people or are not diverse enough. This issue renders fine-tuning models for specific downstream tasks a necessity to ensure the best transcription quality.
The second concern when deploying smaller ASR models is the service quality for a diverse population. Fine-tuning ASR models for specific downstream tasks is often necessary to ensure the best transcription quality, especially for smaller models.
Traditional fine-tuning approaches, such as \citep{survey2024,zaiem2023finetuning,attia2024kidwhisper}, typically fine-tune the model %or employ a single low-rank approximation (LoRA) profile to adapt the model 
to specific tasks or populations with \textit{one single} dataset from the downstream task, under the assumption that the downstream task targets some speakers that share specific similar characteristics. While these methods can enhance performance, they often fall short when dealing with the diverse speech characteristics of a broad population. Such an inability to adjust to a diverse distribution renders those models less practical, which presents the challenge of making the ASR inclusive and fair to a more diverse population.
% ASR models, no matter how big their sizes are, must be inclusive and fair as the real-world scenarios mostly involve speakers from all backgrounds.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{latex/_fig/train_size.png}
%     \caption{Assume each new accent has 1000 training samples. The total training time of existing works scales quadratically in total training size, whereas the proposed P-Whisper only operates on the new data and scales linearly. \textcolor{red}{For now, more beautiful later}}
%     \label{fig:train_size}
% \end{figure}

\input{latex/_table/p-whisper-comparison-model}

Recent works have sought to improve ASR models' ability to accurately transcribe diverse speech by incorporating additional characteristics, mainly accent information, during the training stage \citep{winata2020learning,prabhu2023accented}. Although these approaches have shown effectiveness in improving representation through the additional accent information, they assume a static target distribution. That is, existing works assume a fixed training set with a limited number of accents. When the target distribution evolves with new accents, the entire framework lacks a continual learning ability on the new accents and needs to be retrained, as shown in Table \ref{tab:p-whisper-comparison}. Compared to continual learning, retraining costs quadratic total training time with respect to the data size to ensure catastrophic forgetting does not happen. Moreover, it remains a non-trivial work to add \textit{additional} characteristics besides accents, such as gender or age information, into existing frameworks.
%\amir{We are using the term "fall short" alot}
%In this paper, we consider a practical scenario in which current ASR technologies fall short: how should we maximize the transcription quality if we want to use ASR in a clinical setting, where clinicians use ASR models to help diagnose children with some speech disabilities? In this scenario, the audio samples from children are private and shall not be uploaded to the cloud, which restricts the usage of large ASR models. At the same time, children are from a diverse background and their various characteristics could not be represented very well with a single LoRA profile. On the other hand, it is not possible to use personalized ASR models, such as \textcolor{red}{[cite]}, as there is no training data for each child. Some works try to incorporate 

To address all the aforementioned challenges, we propose \textbf{P-Whisper}, a novel lightweight ASR system that employs multiple LoRA profiles in parallel to fine-tune ASR models and complete downstream tasks. P-Whisper constructs a LoRA profile library for each type of characteristic and structurally identical profiles within each characteristic library. By dynamically selecting and leveraging multiple parallel profiles that accurately represent the speaker's complex background, P-Whisper enables a more nuanced and compelling adaptation process, enhancing transcription quality across a diverse population and improving fairness among marginalized groups. This approach ensures that ASR models remain both high-performing and deployable on local edge devices while maintaining privacy, inclusivity, and operational feasibility. P-Whisper is particularly suited for scenarios where the speaker presents diverse speech characteristics, and those characteristics are not fully available in the training data in the beginning. Ultimately, P-Whisper bridges the gap between advanced ASR capabilities and the practical requirements of real-world applications, offering a robust solution for inclusive and efficient speech recognition.

We summarize our contributions as follows:
\begin{itemize}
    \item We introduce a lightweight ASR framework capable of capturing diverse characteristics of the speakers and utilizing those characteristics to enhance transcription quality.
    \item We demonstrate the effectiveness of merging multiple LoRA profiles for ASR tasks.
    \item We empirically study the performance of P-Whisper, showcasing its superior performance and fairness compared to baselines.
    \item We present the inference latency of utilizing the P-Whisper framework on edge devices, showcasing that off-the-shelf ASR models can achieve near-real-time inference even on resource-constrained devices like the Raspberry Pi.

\end{itemize}

To the best of our knowledge, in addition to the features described in Table \ref{tab:p-whisper-comparison}, compared to similar-size ASR models, P-Whisper achieves state-of-the-art performance on downstream transcription tasks due to its utilization of speaker information. Compared to traditional fine-tuning with a single LoRA profile, P-Whisper's parallel profile framework brings up to 13.7\% relative WER reduction without additional training overhead.


% The rest of the paper unfolds as follows: Section 2 discusses some important background information and the origination of P-Whisper outside of the ASR domain, Section 3 formulates the problem and defines the notations, Section 4 introduces the proposed framework, Section 5 presents the experiments and results, and finally Section 6 concludes the paper. In addition, we provide a discussion of the limitations of the work in Section 7.

==> 1_intro_JX.tex <==
\section{Introduction}

The world has seen significant advancement of artificial intelligence (AI) in the past few years, especially with the arrival of transformer-based foundational models~\cite{}. AI-powered intelligent and personalized agents are becoming more and more of a reality than ever. Since speech is one of the major communication modalities for human's interactions with the environment, automatic speech recognition (ASR) is gaining growing attention from the research community~\cite{}, especially its deployment onto edge devices when privacy is of a great concern~\cite{}. 

The ASR technologies have also experienced tremendous transformation since the introduction of deep neural networks (DNNs). The recent transformer-based ASR models, such as Wave2Vect~\cite{}, Wave2Vect-Comform~\cite{}, and Whisper~\cite{}, have surpassed traditional models like Hidden Markov Models (HMMs) and Gaussian Mixture Models (GMMs) \citep{Povey2011TheKS,Stuttle2003AGM,mcauliffe17_interspeech} in terms of achieving lower word error rates (WERs) and supporting multiple languages simultaneously.
But these transformer-based ASR model sizes are typically large with many parameters,  which require a huge amount of data and computation power to train. Their model inference also requires a significant amount of memory to store the large model parameters. All of these requirements are detrimental for these ASR models' deployment onto resource-constrained edge devices. To address these issues, some recent efforts propose to compress the ASR models for edge deployment through various techniques, such as quantization, pruning, or knowledge distillation. Successful exmamples include Whisper-tiny~\cite{} and WhisperX~\cite{}.

In order for an intelligent agent to truly deliver a personalized experience through ASR, however, three more important considerations must be addressed. (1) The adaptivity of ASR to different speakers' characteristics as different users may have different ways of speaking the same languages. For example, the English speakers' characteristics can be labeled under different categories, such as accents resulting from either cultural or regional differences (such as Black American accents, British accents, or Southern American accents), age-induced speech differences (such as pre-schoolers' speech versus adults' speech), and gender-inherent speech differences (such as male versus female). Ideally, ASR should be adaptive to different speakers' characteristics in order to achieve higher accuracy, and this is especially true for edge-based ASR whose model sizes are constrained by the limited edge resources.  Retraining ASR models from scratch is almost impossible nor feasible as there are just too many variations in terms of speakers' characteristics. (2) The incrementality of ASR to accommodate the ever-evolving interactions among different speakers. For example, the intelligent agent with an ASR trained to understand general American English accents may later encounter situations where interacting with Black American are important as well. However it is still unclear on how to incrementally adding new capabilities to an existing deployed ASR so that it can not only support existing speakers, but also
support the new group of speakers. And (3) the inclusivity of ASR to provide equal and fair experience for speakers with different characteristics. In other words, how can we ensure ASR are not favoring certain groups of population over the others? To the best of our knowledge, none existing edge-based ASR work can meet all the above needs yet.

Therefore, we propose a novel ASR framework, called PI-Whisper, in this work to tackle these three challenges. Our framework is built on an existing ASR backbone, such as Whisper or WhisperX, but augment it with three new components. The first component is a low-rank approximation (LoRA) based fine-tuning module to modify existing ASR's capabilities. The second component is a set of LoRA profiles organized by grouped speaker characteristics. These LoRA profiles can be trained separately from ASR and be added and updated incrementally. The combination of the LoRA component and the LoRA profiles provides a unique opportunity for our ASR to adaptively customize its capabilities based on speakers characteristics. The third component is an automated
identification of speakers' characteristics so that we can optimally choose
the right LoRA profiles for ASR customization. Though each component by itself may not be new, their combination to address the unique edge-ASR issues is novel in our view. Our framework is also inspired in part by the LoRA composition or merging techniques as used in image generation tasks~\cite{}, 
but we are the first one to apply it to ASR to address the above three challenges in a classification task (as compared to an image generation task) to the best of our knowledge. We discuss the details of the proposed PI-Whisper framework and our extensive experimentation. We show that the proposed PI-Whisper framework can not only achieve the state-of-the-art ASR accuracy compared to existing work, but also scales linearly with respect to the required memory sizes and computing power. This is especially appealing for ASR's deployment onto resource-constrained edge devices. So long as the chosen backbone ASR can fit into an edge device, our framework requires minimum additional resources to provide the new capabilities of both adaptivity and incrementality to ASR. More importantly, our framework achieves the highest fairness scores for speakers from different age, gender and accent groups.

The rest of the paper is organized as follows. Section~\ref{sec_background} provides some background about existing work. We formally introduce our problem formulation in Section~\ref{sec_prob} and our framework design
in Section~\ref{sec_design}, respectively. Experimental results will be presented in Section~\ref{sec:experiments}. We conclude the paper in Section~\ref{sec_conclusion} with discussion of our work's limitation in Section~\ref{sec_limits}.



==> 1_intro_v1.tex <==
\section{Introduction}
%\textcolor{red}{NEED to rewrite the story}

The advances in deep learning have brought unprecedented improvement in the field of automatic speech recognition (ASR). Recent works such as \cite{radford2022robust,rekesh2023fast,bain23_interspeech} have demonstrated remarkable accuracy and robustness in recognizing speech across various languages, accents, and noisy environments. However, despite these advancements, there remain significant challenges in adapting these models to diverse populations, particularly when considering the computational constraints of deployment on edge devices.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{latex/_fig/librispeech.png}
    \caption{Different sizes of Whisper model's performance on Librispeech (clean) dataset's test split.}
    \label{fig:libri}
\end{figure}

One of the foremost practical challenges in ASR today is the balance between model accuracy and deployment feasibility. Arguably, transformer models more-or-less all follow the scaling law \citep{kaplan2020scaling}, which states that the performance of a model is positively related to its size. In ASR, larger models typically yield better performance due to their capacity to capture complex linguistic patterns and variations. As shown in Figure \ref{fig:libri}, the performance of different variations of the Whisper family \citep{radford2022robust} on two benchmarks \citep{librispeech, Heikinheimo_2023} indicates that larger models achieve higher quality transcriptions with lower word error rates (WER). 

Nonetheless, in scenarios where the privacy of training and inference data is valued, these large and powerful models are often too resource-intensive to be deployed on local edge devices, which have limited computational power and resources \citep{qin2024empirical}. For example, when the ASR tasks involve transcribing and analyzing audio samples from sensitive subjects who do not wish to disclose their speech \citep{ahmed2020preech,liu2022private}, large ASR models that are running on cloud computation infrastructures could not be used, and we will have to consider smaller models that are not as expressive yet fit into edge devices. 

%\amir{We need to emphasize the use case of edge more}

When deploying smaller ASR models, fine-tuning them for specific downstream tasks is often necessary to ensure the best transcription quality. Traditional fine-tuning approaches, such as \citep{survey2024,zaiem2023finetuning,attia2024kidwhisper}, typically fine-tune the model %or employ a single low-rank approximation (LoRA) profile to adapt the model 
to specific tasks or populations with \textit{one single} dataset from the downstream task, under the assumption that the downstream task targets some speakers that share certain similar characteristics. While these methods can enhance performance, they often fall short when dealing with the diverse speech characteristics of a broad population. Such an inability to adjust to a diverse distribution renders those models less practical, as the real-world scenarios mostly involve speakers from all backgrounds.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{latex/_fig/train_size.png}
    \caption{Assume each new accent has 1000 training samples. The total training time of existing works scales quadratically in total training size, whereas the proposed P-Whisper only operates on the new data and scales linearly. \textcolor{red}{For now, more beautiful later}}
    \label{fig:train_size}
\end{figure}

Recent works have sought to improve ASR models' ability to accurately transcribe diverse speech by incorporating additional characteristics, mainly accent information, during the training stage \citep{winata2020learning,prabhu2023accented}. Although these approaches have shown effectiveness in improving representation through the additional accent information, they assume a static target distribution. That is, existing works assume a fixed training set with a limited number of accents, and when the target distribution evolves with new accents, the entire framework needs to be retrained. As shown in Figure \ref{fig:train_size}, retraining on the existing framework costs quadratic total training time with respect to the data size to ensure catastrophic forgetting does not happen. Moreover, it remains a non-trivial work to add \textit{additional} characteristics besides accents, such as gender or age information, into existing frameworks.
%\amir{We are using the term "fall short" alot}
%In this paper, we consider a practical scenario in which current ASR technologies fall short: how should we maximize the transcription quality if we want to use ASR in a clinical setting, where clinicians use ASR models to help diagnose children with some speech disabilities? In this scenario, the audio samples from children are private and shall not be uploaded to the cloud, which restricts the usage of large ASR models. At the same time, children are from a diverse background and their various characteristics could not be represented very well with a single LoRA profile. On the other hand, it is not possible to use personalized ASR models, such as \textcolor{red}{[cite]}, as there is no training data for each child. Some works try to incorporate 

To address these challenges, we propose \textbf{P-Whisper}, a novel ASR framework that employs multiple LoRA profiles in parallel to fine-tune ASR models and complete downstream tasks. This method is particularly suited for scenarios where the speaker presents diverse speech characteristics, and those characteristics are not fully available in the training data in the beginning. By leveraging multiple parallel profiles, P-Whisper enables a more nuanced and effective adaptation process, enhancing transcription quality across a diverse population. This approach ensures that ASR models remain both high-performing and deployable on local edge devices, maintaining privacy and operational feasibility. Ultimately, P-Whisper bridges the gap between advanced ASR capabilities and the practical requirements of real-world applications, offering a robust solution for inclusive and efficient speech recognition.

The rest of the paper unfolds as follows: Section 2 discusses some important background information and the origination of P-Whisper outside of the ASR domain, Section 3 formulates the problem and defines the notations, Section 4 introduces the proposed framework, Section 5 presents the experiments and results, and finally Section 6 concludes the paper. In addition, we provide a discussion of the limitations of the work in Section 7.

==> 5_discussions.tex <==
\section{Discussions}

==> 6_limitations.tex <==
\section{Limitations}
\label{sec_limits}
We recognize several limitations of our work. Some of the limitations are on areas of less importance and we choose not to experiment and elaborate, and some of them are due to resource limitations.
\begin{enumerate}
    \item We do not discuss the classifier's potential quadratic retraining cost. Since the classifier is a CNN structure, the retraining/adaptation cost can be linear with continual learning and incremental learning. There is a rich literature on this subject, such as \citep{incremental2024}, but that requires additional work over what we present in the paper.
    \item We do not discuss the weights for merging the LoRA profiles. In the paper, we assume it is $\frac{1}{K}$ and use the same number throughout the experiments. However, there exist more advanced methods of selecting the merging weights, such as \citet{wu2024mixture}.
    \item This work is not about optimizing the classifier for different characteristics. We just choose a reasonable network that has decent performance. We believe that the accuracy of the classifier could be higher, but we choose not to work on that in this paper.
    \item We choose to use a fixed seed (42) for everything and only run the experiments once. We acknowledge that a better way is to run the experiments multiple times and report the average and variance, but due to resource constraints (GPU), we are not able to conduct experiments with multiple trials.
    \item We conduct experiments with one model and two datasets. It would be good if we could conduct more experiments on other models and datasets, but we did not do so due to resource constraints, similar to the reason above.
\end{enumerate}





==> __problem.tex <==
\section{Problem Formulation}
\label{sec_prob}

We focus on developing an ASR inference framework on edge devices toward two similar downstream tasks with a non-static distribution that is different from the pre-training dataset. For ease of discussion, we will refer to the first downstream task as the Anonymous setting, where we do not have access to the speaker's identity, and we will refer to the other variation as the Identified setting, where the speaker's identity is known during inference. In this section, we formally define the considered problem and elaborate on the two settings.

\subsection{Anonymous Setting}
In this setting, we consider a framework $M$ that contains some pre-trained ASR model on some generic distribution $D$ which consists of many audio and transcription pairs. We formalize $D$ as $D=\{(a_1,t_1),...\}$, where $a$ is the audio sample and $t$ is its corresponding transcription. In addition, we consider a downstream distribution that is diverse and non-static, denoted as $D' = \{(a_1',t_1',c^1_1,c^2_1,...,c^k_1),...\}$, where $c_i^k \in C^{k}$ represents that the characteristic of the speaker is one of the possible choices in the characteristic set $C^{k}$, which represents all potential characteristics of that type. Common characteristics include the accent, gender, and age of the speaker. In addition, the downstream task's distribution is non-static with an increasing complexity. In the beginning, we might not be aware of all the choices in the true characteristic set, $C^{k+}$. Formally, we say that when we initially fine-tune $M$, our available dataset is $D' \subset D'^+$, where $d_i \in D' = (a_i',t_i',c^1_i,c^2_i,...,c^k_i)$, and $C^k \subset C^{k+}$. As time goes on, $D'$ expands to $D'^+$, which is the result of $C^k$ expanding and evolving towards $C^{k+}$. After expansion, for each training sample $d_i$, $c^k_i \in C^{k+}$.
%the sample within the downstream distribution takes the form of $d \in D'^+ = (a_1',t_1',c^1_1,c^2_1,...,c^k_1)$, where $c^k_1 \in C^{k+}$.

In order to maximize the accuracy of $M$ on $D'^+$, we use whatever dataset at hand to perform fine-tuning. That is, we initially fine-tune $M$ with $D'$ and seek opportunities to update $M$ as $D'$ expands.
During the inference stage, the Anonymous setting considers an input sample $s_i = (a_i')$, where $s_i \in D'^+$. Under this setting, we only get the audio sample during inference, and our goal is to get the accurate transcription, which could be denoted as $\min \textit{WER}[M(a_i'),t_i']$.


\subsection{Identified Setting}

The Identified setting is the same as the Anonymous setting during fine-tuning, but it additionally assumes the knowledge of the speaker's identity during inference. That is, it considers the input sample as $s_i = (a_i', c^1_i, c^2_i, ...,c^k_i)$, and a similar objective needs to be achieved: $\min \textit{WER}[M(a_i',c^1_i, c^2_i, ...c^k_i),t_i']$. We argue that while most existing works focus on the variations of ASR under Anonymous settings, the Identified setting is also achievable under certain scenarios. In particular, in most private settings where the ASR model is more of an assistant tool over a service, it is not hard to obtain the ground truth of the speaker's characteristics $(c^1_i,c^2_i...,c^k_i)$ beforehand.


==> __theory.tex <==
\section{Theoretical Analysis: what is the optimal solution to a diverse population?}

In this section, we provide mathematical analyses of the gradient descent of a DL model on a diverse population. In particular, we focus on two important insights that are the fundamentals of the proposed framework. 

\subsection{Separate vs. Unified finetuning}
\label{sec:theory}
In this subsection, we investigate the effect of splitting a diverse population according to some characteristics, and we will prove that such a practice will lead to a lower loss compared to performing the gradient descent on the entire population. The analysis will be presented in two ways.

First, the loss from the gradient descent process is analyzed. For simplicity of proof, we take the categorical cross-entropy loss (which is the standard loss in ASR tasks), but the proof generalizes to other losses. It is additionally assumed that the diverse population D can be divided according to some characteristics $C^k$, and different characteristics (e.g. Irish vs. Canadian accent) have some different features. The cross-entropy loss of dataset D is defined as:

\begin{equation}
    CE(D) = - \sum_{d_i\in D} t_i log(M(a_i))
\end{equation}

However, if we split D into different groups according to some characteristics, we have $D=\{D^1,D^2, D..., D^{|C^k|}\}$. The concrete examples of such a split can be seen in Equation \ref{eq.1}. For each $D^l$, we have its loss as:
\begin{equation}
    CE(D^l) = - \sum_{d_i \in D^l} t_i log(M(a_i)) %\forall (a_i,t_i \in D^l)
\end{equation}

Since the union of all $D^l$ is $D$, by construction, the loss of $D$ can also be written as:

\begin{equation}
    CE(D) = - \sum_{l=1}^{|C^k|}\sum_{d_i \in D^l} t_i log(M(a_i)) % \forall (a_i,t_i \in D^l)
\end{equation}

The gradient descent of some weight $w$ in the model $M$ on $CE(D)$ can be written as:
\begin{equation}
    w' = w+ \eta \nabla_w CE(D) = w - \eta \nabla_w \sum_{l=1}^{|C^k|}\sum_{d_i \in D^l} t_i log(M(a_i)) % \forall (a_i,t_i \in D^l)
\end{equation}

It is not hard to see that compared to training on $D^l$, $\nabla_w$ reaches 0 (model converges) earlier on $D$. This is because all features shared by samples in $D$ exist in $D^l$, but $D^l$ contain individualized characteristic features that are not consistent in $D$. Formally, during the gradient descent process, we will have the following scenario on characteristic-specific features:
\begin{equation}
\begin{aligned}
       w'& = w+ \eta \nabla_w CE(D) \\&= w - \eta [\underbrace{\nabla_w \sum_{d_i \in D^l} t_i log(M(a_i)) }_{\textit{positive gradient}} 
    + \underbrace{\nabla_w \sum_{d_i \in D-D^l} t_i log(M(a_i))}_{\textit{negative gradient}}] 
\end{aligned}
\end{equation}
% \begin{equation}
% \begin{aligned}
%     w' &= w + \eta \nabla_w CE(D) \\
%     &= w - \eta \left[ \underbrace{\nabla_w \sum_{d_i \in D^l} t_i \log(M(a_i))}_{+} 
%     + \underbrace{\nabla_w \sum_{d_i \in D-D^l} t_i \log(M(a_i))}_{-} \right]
% \end{aligned}
% \end{equation}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth,trim={2.03cm 2.85cm 1.6cm 3cm},clip]{_fig/2d_illus.png}
    \caption{Gradient Descent Illustration}
    \label{fig:2d_illus}
\end{figure}
Similarly, this phenomenon can also be shown through the gradient vector's direction. Assuming the features of different characteristics do not align perfectly with each other, then optimizing $M$ on $D$ is less optimal compared to optimizing $M$ on each $D_l$ separately. As illustrated in Figure \ref{fig:2d_illus}, when the samples belonging to two characteristics have different features, the gradient descent direction will be different. Training on a uniform dataset containing both groups of samples will lead to a suboptimal optimization direction for both of the groups.



\subsection{Samples Multiple Characteristics}

We have shown that it is better to fine-tune a model according to some characteristic ($C^k$) of the dataset to achieve minimal loss. However, it is yet unclear what to do when multiple characteristics exist in a population. As discussed in the related works, other areas have shown that merging LoRA adapters is useful. Here, we discuss the different ways of merging the LoRA and provide an intuitive explanation of using the LoRA merging technique.

Typically, when there are only LoRA adapters existing, there are three ways of merging them, namely concatenation (Equation \ref{eq:concat}), linear (Equation \ref{eq:linear}), and SVD (taking SVD of Equation \ref{eq:concat}).
\begin{equation}
    W'(x) = W(x) + [ \bigoplus_{k=1}^{|\mathbf{C}|} w_k B_k \cdot\bigoplus_{k=1}^{|\mathbf{C}|} w_k A_k](x)
    \label{eq:concat}
\end{equation}

\begin{equation}
    W'(x) = W(x) + [ \sum_{k=1}^{|C|} \sqrt{w_kB_k} \sum_{k=1}^{|C|} \sqrt{w_kA_k}](x)
    \label{eq:linear}
\end{equation}



In the equation, $W'(x)$ is the output from a layer with LoRA adaptation, $W(x)$ is the output from a layer calculated with weights from the base model, $w_j$ is the hyperparameter that controls the strength of the LoRA profile, where we follow the convention and set to be $\frac{1}{|\mathbf{C}|}$, and $B_kA_k$ is the LoRA decomposition. The $\bigoplus$ is the concatenation symbol, and the decomposition matrices of LoRA are concatenated respectively before multiplication.

Compared to a single LoRA adapter, using multiple LoRA has two advantages. First, according to the scaling law \cite{kaplan2020scaling}, more parameters generally mean more accurate models. \footnote{Although the scaling law was originally studied with LLMs, it generalizes to all transformer structure models.} More LoRA adapters mean more parameters to adjust to the nuanced features from the training set, which leads to better performance after merging. Second, similar to the illustration of splitting the dataset according to single characteristics in Figure \ref{fig:2d_illus}, if a sample contains multiple characteristics that have different gradient descent directions, training using only one characteristic (the green arrow) will not represent the features from the other characteristic (the red arrow). Merging the adapters of two characteristics will land the model in a middle state (the blue arrow) and better represent the characteristics of the specific sample.

In the end, we briefly discuss why concatenation works best in the general case. it can be seen that the linear approach takes an additional square root on the weights. Such practice might be useful as a normalization technique, but it might also lead to an amplification or suppression of some important weights. The SVD approach takes an approximation of the merged adapters. It might be useful to pick up important features, but it also loses information. Concatenation preserves all information in the original state and intuitively works best in the general case. We also empirically show that in Table \ref{tab:wer_methods}.

\input{_table/merge}

==> _table/dataset.tex <==
\begin{table}[h]
\centering
\tabcolsep 17pt
\caption{Number of grouped speaker characteristics.
%Number of profiles (characteristics) in each LoRA profile library. 
}
\begin{tabular}{|c|ccc|}
\hline
            & \multicolumn{3}{c|}{Speaker Characteristics}                             \\ \cline{2-4}
Dataset     & \multicolumn{1}{c|}{Gender} & \multicolumn{1}{c|}{Accent} & Age \\ \hline
L2-Arctic   & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{6}      & --  \\
CommonVoice & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{5}    & 9   \\ \hline
\end{tabular}

\label{tab:dataset}
\end{table}

==> _table/merge.tex <==
% \begin{table}[h]
%     \centering
    
%     \begin{tabular}{|c|c|}
%          \hline
%         \textbf{Method} & \textbf{WER (\%)} \\
%          \hline
%         SVD & 25.35 \\
%         Linear & 18.71 \\
%         Concat & 17.45 \\
%          \hline
%     \end{tabular}
%  \caption{Word Error Rate (WER) for Different Methods of Merging Gender and Age Lora libraries on L2-Arctic}
%     \label{tab:wer_methods}
% \end{table}

\begin{table}[h]
    \centering
     \caption{Word Error Rate (WER) for Different Methods of Merging Gender and Age Lora libraries on L2-Arctic}
    \begin{tabular}{|c|c|}
         \hline
        \textbf{Method} & \textbf{WER (\%)} \\
         \hline
        \makebox[4cm]{\centering SVD} & \makebox[2.5cm]{\centering 25.35} \\
        \makebox[4cm]{\centering Linear} & \makebox[2.5cm]{\centering 18.71} \\
        \makebox[4cm]{\centering Concat} & \makebox[2.5cm]{\centering 17.45} \\
         \hline
    \end{tabular}
    \label{tab:wer_methods}
\end{table}









% \begin{table}[h]
%     \centering
% \begin{tabular}{|lr|}
% \hline
% \multicolumn{1}{|l|}{Method} & \multicolumn{1}{l|}{WER} \\ \hline
% SVD                          & 25.35                    \\
% Linear                       & 0.1871                   \\
% concat                       & \textbf{0.1745}          \\ \hline
% \end{tabular}
% \label{tab:wer_methods}
%  \caption{Word Error Rate (WER) for Different Methods of Merging Loras}
% \end{table}
